Adding Safety Rules to Surgeon-Authored VR Training

Introduction: Safety criteria in surgical VR training are typically hard-coded and informally summarized. The Virtual Reality (VR) content creation interface, TIPS-author, for the Toolkit for Illustration of Procedures in Surgery (TIPS) allows surgeon-educators (SEs) to create laparoscopic VR-training modules with force feedback. TIPS-author initializes anatomy shape and physical properties selected by the SE accessing a cloud data base of physics-enabled pieces of anatomy. Methods: A new addition to TIPS-author are safety rules that are set by the SE and are automatically monitored during simulation. Errors are recorded as visual snapshots for feedback to the trainee. This paper reports on the implementation and opportunistic evaluation of the snap-shot mechanism as a trainee feedback mechanism. TIPS was field tested at two surgical conferences, one before and one after adding the snapshot feature. Results: While other ratings of TIPS remained unchanged for an overall Likert scale score of 5.24 out of 7 (7 equals very useful), the rating of the statement `The TIPS interface helps learners understand the force necessary to explore the anatomy' improved from 5.04 to 5.35 out of 7 after the snapshot mechanism was added. Conclusions: The ratings indicate the viability of the TIPS open-source2 E-authored surgical training units. Presenting SE-determined procedural missteps via the snapshot mechanism at the end of the training increases acceptance

==> intro.tex <==
\section{Introduction}
Assessment is a critical component in the training of novice surgeons.
Assessment of surgical proficiency has two components: 
verifying that certain milestones are achieved and 
avoiding surgical errors. 
Assessment in the workplace is typically time intensive and stressful 
as it requires an experienced surgeon instructor to be both present and  
possibly intervene at moment's notice. 
To make the assessment more objective, a majority of programs now employ 
objective structured assessment of technical skills
(OSATS) for workplace-based assessment \cite{osats:}


Conversely, assessment is a central part of computer games.
Here simple counters for the 
game character picking up `treasures' and progressing towards a next level 
while avoiding perils are classic tools of the trade. 
Psychometric games even claim to measure mental agility, attention, 
cognitive speed, spatial aptitude and numerical processing ability.

%SimCity SuperMario 
%But one of the most common misconceptions we have run across is that all good learning games must assess learners within the game. The truth is that assessment happens around a game more often than it happens inside the game, and teachers must still design and provide authentic, useful assessment tasks for students.

We encountered the challenge of assessing laparoscopic safety 
proficiency in the context of developing an environment that allows
surgeon-educators to author laparoscopic VR-training modules
with force feedback.
This authoring environment, 
the Toolkit for Illustration of Procedures in Surgery (TIPS) 
consists of TIPS-simulator, an interactive soft-tissue laparoscopic
simulation, TIPS-trainee, providing instruction and examples and 
TIPS-author, an interface  that allows the surgeon-educator
to specify steps of a minimally invasive procedure in the fixed format:
action, anatomy, tool, safety, comment (see \figref{})
The entries `action, anatomy, tool' initialize the anatomy 
and its physical properties with respect to the tools
\cite{Saleh}. The key to this high-level initialization of scenarios
by the surgeon-educator is to accumulate a rich database of 
physically annotated and compatible anatomy, so called simlets.
Simlets are created by content artists, and can be combined in a
lego-like fashion. The web-based TIPS-author interface \cite{recent}
provides a auto-completion for items recognized to be in the database
and thereby steers the author towards existing simlets.

Our challenge is the `safety' entry in the TIPS-author sepcification 
of a surgical task. This entry is to provide a palette of surgical 
safety criteria such as: not cauterizing near sensitive organs or
limiting the application of force when mobilizing vessels from
fatty tissue before clamping. 
While on one hand, haptic interactive simulation is no different from
(a specialized) computer game, on the other hand the challenge 
differs in that the assessment criteria can not be hard-coded a priori 
as in a game environment because the surgeon-author sets the criteria.
The goal is to insure that \emph{surgical safety criteria}
can be formulated, automatically translated into measurable events during VR 
simulation and presented to the trainee both as immediate
feedback and final report to be shared with the instructor.


This paper reports on an approach 
\begin{enumerate}
\item
that allows the surgeon-educator to specify surgical safety criteria
\item
that are automatically instantiated 
\item
that are automatically monitored within TIPS-simulator 
(without requiring trainee and instructor to be 
present or engaged at the same time)
\item
that provides immediate feedback to the trainee
\item
and a summative feedback in a secure fashion
both the trainee and  
\item
as an automatic report to the instructor, listing errors  or 
confirming proficiency with respect to the unit.
\end{enumerate}

Naturally the approach is greatly aided by restricting the 
vocabulary to the surgical task. For example, sensitive organs are organs 
in the database and the majority of criteria fall into three
categories that we identified as:  proximity, force application
and clamping/stapling layout.

\paragraph{Overview}
%A novel Virtual Reality (VR) content creation interface allows
%As front-end to the 


